Template Matching with Deformable Diversity Similarity

We propose a novel measure for template matching named Deformable Diversity Similarity -- based on the diversity of feature matches between a target image window and the template. We rely on both local appearance and geometric information that jointly lead to a powerful approach for matching. Our key contribution is a similarity measure, that is robust to complex deformations, significant background clutter, and occlusions. Empirical evaluation on the most up-to-date benchmark shows that our method outperforms the current state-of-the-art in its detection accuracy while improving computational complexity.

==> BBS.tex <==
\section{Review of Best-Buddies Similarity (BBS)} 
\label{sec:BBS}


The BBS proposed in~\cite{dekel2015best} measures the similarity between two sets of points $P\!=\!\{p_i\}_{i=1}^{N}$ and $Q\!=\!\{q_i\}_{i=1}^{M}$, where $p_i,q_i \in \mathbb{R}^d$.
The BBS is the fraction of \emph{Best-Buddies Pairs} (BBP) between the two sets. Specifically, a pair of points $\{p_i{\in}P , q_j{\in}Q \}$ are called a BBP if $p_i$ is the Nearest Neighbor (NN) of $q_j$, and vice versa. Formally,
\begin{equation}
\label{eq:BBS}
\textbf{BBS}(P,Q)=\frac{1}{\min{\{M,N\}}}\cdot\sum_{p_i{\in}P}\sum_{q_j{\in}Q}{bb_{i,j}(P,Q)}
\end{equation}
%
where $bb_{i,j}(P,Q)$ is the best buddies pair indicator:
\begin{equation}
\label{eq:bbij}
bb_{i,j}(P,Q) =
\begin{dcases*}
\begin{array}{ll}
1\! &\! \mathrm{NN}(p_i,Q)\!=q_j\! \wedge\! \mathrm{NN}(q_j,P)\!=p_i\!\\
0\! &\!\text{otherwise}
\end{array}
\end{dcases*}
\end{equation}
%
Here $\mathrm{NN}(p_i,Q)=\argmin_{q{\in}Q}d(p_i,q)$ for some distance measure $d(p_i,q)$, typically the Euclidean distance. 

%To detect a given template $T$ in a target image $S$ the traditional sliding window approach is used. The BBS is computed between the template  $T$ and every possible window $W$ (of the size of the template) in the image. This is done by breaking every window into distinct non-overlapping patches of fixed dimension.


%BBS possesses several properties that make it attractive: 
%1) it relies only on a subset of matches, i.e., pairs of points that are BBPs, whereas the rest are considered as outliers. 
%2) BBS does not require any prior knowledge on the data or its underlying deformation.
%3) BBS uses rank, i.e., it counts the number of BBPs, rather than using the actual distance values.
%As was shown in~\cite{dekel2015best}, these properties allow BBS to overcome several significant challenges such as background clutter, occlusions, and nonrigid deformation of the object. Indeed, the template matching results of BBS are superior to all previous methods.
%
%One limitation of BBS for template matching is its computational complexity. Since it requires finding the NNs both in $P$ and in $Q$ these have to be re-computed for every target window. To make the computation of BBS tractable~\cite{dekel2015best} extract only distinct, non-overlapping patches from both target and template. 



==> DIS_bounds_BBS.tex <==
\paragraph{DIS bounds BBS}

\begin{claim}
\begin{equation}
\label{eq:DIS-bounds-BBS}
\underset{P,Q}{{\textbf{BBS}}}  \leq \quad \min\left\{
\underset{Q{\rightarrow}P}{{\textbf{DIS}}},
\underset{P{\rightarrow}Q}{{\textbf{DIS}}}
\right\}
\end{equation}
\end{claim}
%
\begin{claimproof}
To prove this claim we start by providing definitions of BBS and DIS as sums of contributions over the points in $P$.
The contribution of a point $p_i{\in}P$ to BBS and DIS can be formulated as follows:
%
\begin{equation}
\label{eq:bbsi}
bbs_{i}(Q,P) =
\\
\begin{dcases*}
\begin{array}{lll}
\multirow{2}{*}{1}\! &\! {\exists}q_j{\in}Q,\\ 
	&\! \mathrm{NN}(q_j,P)\!=p_i \wedge \mathrm{NN}(p_i,Q)\!=q_j\\
0\! &\!\text{otherwise}
\end{array}
\end{dcases*}
\end{equation}
%
\begin{equation}
\label{eq:disi}
dis_{i}(Q,P) =
\begin{dcases*}
\begin{array}{ll}
1\! &\! {\exists}q_j{\in}Q ,\mathrm{NN}(q_j,P)\!=p_i\!\\
0\! &\!\text{otherwise}
\end{array}
\end{dcases*}
\end{equation}
%
We can now write BBS and DIS as sums of contributions:
%
\begin{equation}
\underset{P,Q}{{\textbf{BBS}}}=\frac{1}{\min{\{M,N\}}} \sum_{i=1}^{N}{bbs_{i}(Q,P)}
\end{equation}
\begin{equation}
\underset{Q{\rightarrow}P}{{\textbf{DIS}}}=\frac{1}{\min{\{M,N\}}} \sum_{i=1}^{N}{dis_{i}(Q,P)}
\end{equation}
%
From the definitions in~\eqref{eq:bbsi} and~\eqref{eq:disi} we immediately have:
%
\begin{equation}
\big(bbs_{i}(P,Q)=1\big) \quad {\Longrightarrow} \quad \big(dis_{i}(P,Q)=1\big)
\end{equation}
%
Thus we can deduce that:
%
\begin{equation}
\underset{P,Q}{{\textbf{BBS}}} \leq \underset{Q{\rightarrow}P}{{\textbf{DIS}}}
\end{equation}
%
Finally, using the fact that BBS is symmetric in $P$ and $Q$, swapping the roles of $P$ and $Q$ results in~\eqref{eq:DIS-bounds-BBS} which completes the proof.
\end{claimproof}

Going back to Figure~\ref{fig:ExpectationAnalysis}, it is now clearer why the expectation of DIS and BBS are so similar.

==> fig_example.tex <==
\fboxsep=0mm%padding thickness
\fboxrule=1.5pt%border thickness
\begin{figure}
		\centering
		\rotatebox{90}{\hspace{0.1cm}}~
		\vspace{0.1cm}
		\begin{subfigure}[b]{.14\textwidth}\fcolorbox{CornflowerBlue}{yellow}{\includegraphics[width=.98\linewidth]{Intro/imageExamples/womanT.png}}\end{subfigure}~
		\begin{subfigure}[b]{.14\textwidth}\fcolorbox{CornflowerBlue}{yellow}{\includegraphics[width=.98\linewidth]{Intro/imageExamples/runnerT.png}}\end{subfigure}~
		\begin{subfigure}[b]{.14\textwidth}\fcolorbox{CornflowerBlue}{yellow}{\includegraphics[width=.98\linewidth]{Intro/imageExamples/dollT.png}}\end{subfigure}
		\rotatebox{90}{\hspace{0.1cm}}~
		\vspace{0.1cm}
		\begin{subfigure}[b]{.14\textwidth}\fcolorbox{green}{yellow}{\includegraphics[width=.98\linewidth]{Intro/imageExamples/womanS.png}}\end{subfigure}~
		\begin{subfigure}[b]{.14\textwidth}\fcolorbox{green}{yellow}{\includegraphics[width=.98\linewidth]{Intro/imageExamples/runnerS.png}}\end{subfigure}~
		\begin{subfigure}[b]{.14\textwidth}\fcolorbox{green}{yellow}{\includegraphics[width=.98\linewidth]{Intro/imageExamples/dollS.png}}\end{subfigure}
     	\rotatebox{90}{\hspace{0.1cm}}~
		\vspace{0.1cm}
        \begin{subfigure}[b]{.215\textwidth}\fcolorbox{CornflowerBlue}{yellow}{\includegraphics[width=.98\linewidth]{Intro/imageExamples/bikeT.png}}\end{subfigure}~
        \begin{subfigure}[b]{.215\textwidth}\fcolorbox{green}{yellow}{\includegraphics[width=.98\linewidth]{Intro/imageExamples/bikeS.png}}\end{subfigure}
	\caption{ \textbf{Template matching challenges:}  The template objects are marked by blue bounding boxes on the template images (blue frame); The best matches are marked by green bounding boxes over the target images (green frame). Images are taken from \cite{dekel2015best,wu2013online}. Different challenges are evident: the journal occludes the woman's face, the runner moves non-rigidly, the doll undergoes out-of-plane rotation, and the motorcyclist shows both a large portion of changing background as well as a complex deformation.
\lihi{I don't like this figure. I think that instead we can take the second example from Figure 7 (of the basketball player). That example shows occlusion, rotation, and deformation.}	
	}
	\label{fig:templateMatchingEx}
\end{figure}

==> fig_nnf.tex <==
\begin{figure}[t]
\captionsetup[subfigure]{labelformat=empty}
    \begin{center}
	\includegraphics[width=.9\linewidth]{NNF.png}
        \vspace{-5pt}
	\end{center}
    \vspace{-0.3cm}
	\caption{\textbf{The NN field:} 
	Given a target image $S$ we find for each point $q_j$ its NN in the template, in terms of appearance: $p_i\!=\!\mathrm{NN}^a(q_j,P)$ where $P$ is the set of features in $T$ and $p_i{\in}P$.
The dashed square marks the position of $p_i$ in the coordinate system of a target sub-window $W$. The dashed arrow $(u_j,v_j)$ marks the displacement vector between the positions $p_i^l$ and $q_j^l$ with length $r_j=||(u_j,v_j)||_2$.}
\vspace{-0.3cm}
\label{fig:nnf}
\end{figure}

==> fig_th.tex <==
\begin{figure}[ht]
		\centering
		\rotatebox{90}{\hspace{0.1cm}}~
		\vspace{0.1cm}
		 \begin{subfigure}[b]{.14\textwidth}\includegraphics[width=.98\linewidth]{th/a.jpg}\caption{input image}\end{subfigure}~
		\begin{subfigure}[b]{.14\textwidth}\includegraphics[width=.98\linewidth]{th/b.jpg}\caption{optimal $\tau$}\end{subfigure}~
		\begin{subfigure}[b]{.14\textwidth}\includegraphics[width=.98\linewidth]{th/c.jpg}\caption{high $\tau^{+}$}\end{subfigure}
		\caption{\textbf{Find the optimal $\tau$.} \textcolor[rgb]{1,0,0}{TODO}.}
		\label{fig:th}
\end{figure}

